Semantic Segmentation with Generative Models: Semi-Supervised Learning and Strong Out-of-Domain Generalization

Training deep networks with limited labeled data while achieving a strong generalization ability is key in the quest to reduce human annotation efforts. This is the goal of semi-supervised learning, which exploits more widely available unlabeled data to complement small labeled data sets. In this paper, we propose a novel framework for discriminative pixel-level tasks using a generative model of both images and labels. Concretely, we learn a generative adversarial network that captures the joint image-label distribution and is trained efficiently using a large set of unlabeled images supplemented with only few labeled ones. We build our architecture on top of StyleGAN2, augmented with a label synthesis branch. Image labeling at test time is achieved by first embedding the target image into the joint latent space via an encoder network and test-time optimization, and then generating the label from the inferred embedding. We evaluate our approach in two important domains: medical image segmentation and part-based face segmentation. We demonstrate strong in-domain performance compared to several baselines, and are the first to showcase extreme out-of-domain generalization, such as transferring from CT to MRI in medical imaging, and photographs of real faces to paintings, sculptures, and even cartoons and animal faces. Project Page: \url{https://nv-tlabs.github.io/semanticGAN/}

==> figures/results/ablation.tex <==
\begin{figure}[t!]
\vspace{-2mm}
\begin{adjustbox}{width=0.82\linewidth,center}
\begin{tabular}{cc}
\includegraphics[width=0.46\linewidth]{figures/ablation/face-full-ood-stepvsmiou.pdf}
&
\includegraphics[width=0.46\linewidth]{figures/ablation/face-full-ood-lpipsvsmiou.pdf}
\end{tabular}
\end{adjustbox}
\vspace{-4mm}
\caption{\footnotesize \textbf{Ablation Study on optimization hyperparmeters}, on the  Metface dataset trained using 1500 Celeba-Mask Labels. Here $\lambda$ is the $\lambda_2$ as in Eq (~\ref{eq:testtime_opt}). Optimization improves performance even with small steps, performance peaked at certain steps. High reconstruction quality (low score in LPIPS) correlated to high task performance. }
\label{fig:qual}
\vspace{-2mm}
\end{figure}

==> figures/results/ct_results.tex <==
\begin{figure*}[h!]
%\begin{minipage}{0.47\linewidth}
\begin{adjustbox}{width=0.8\linewidth, center}
\footnotesize
\addtolength{\tabcolsep}{-4pt}
\begin{tabular}{cccccccc}
& image & GT  & DeepLab& MT&AdvSSL& GCT &Ours \\
%
%% \multicolumn{2}{c}{Synthesized Skin Lesion and Label} &
% \multicolumn{2}{c}{Synthesized Liver CT and Label} 
% \multirow{1}{*}{\rotatebox[origin=c]{90}{In-Domain}}
\rotatebox{90}{\scriptsize \hspace{-1mm}In-Domain}
% &
% \includegraphics[width=0.125\linewidth]{figures/cxr/JSRT/test-img/JPCLN003.png}
% &
% \includegraphics[width=0.125\linewidth]{figures/cxr/JSRT/test-gt/JPCLN003_pred.png}

% &
% \includegraphics[width=0.125\linewidth]{figures/cxr/JSRT/deeplab/JPCLN003.png_1351_50_labeled2-pred_convert.png}
% &
% \includegraphics[width=0.125\linewidth]{figures/cxr/JSRT/sslmt/JPCLN003.png_1431_50_teacher2-pred_convert.png}
% &
% \includegraphics[width=0.125\linewidth]{figures/cxr/JSRT/ssladv/JPCLN003.png_251_50_labeled2-pred_convert.png}
% &
% \includegraphics[width=0.125\linewidth]{figures/cxr/JSRT/sslgct/JPCLN003.png_1181_50_l2-pred_convert.png}
% &
% \includegraphics[width=0.125\linewidth]{figures/cxr/JSRT/ours/JPCLN003_pred.png}
% \\
&
\includegraphics[width=0.125\linewidth]{figures/lits/indomain/test-img/volume-32_0090.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/indomain/test-gt/volume-32_0090.png}

&
\includegraphics[width=0.125\linewidth]{figures/lits/indomain/deeplab/volume-32_0090_pred.png_3_1109_labeled2-pred_pred.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/indomain/mt/volume-32_0090_pred.png_7_1109_teacher2-pred_pred.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/indomain/advssl/volume-32-0090.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/indomain/gct/volume-32_0090.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/indomain/ours/volume-32_0090.png}
\\
\multirow{2}{*}{\rotatebox[origin=c]{90}{MR-T1-in}}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/test-img/volume_0002_0020.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/test-gt/volume_0002_0020.png}

&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/deeplab/volume_0002_0020_pred.png_3_122_labeled2-pred_pred.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/mt/volume_0002_0020_pred.png_7_122_teacher2-pred_pred.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/advssl/volume_0002_0020.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/gct/volume_0002_0020.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/ours/volume_0002_0020.png}
\\
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/test-img/volume_0006_0015.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/test-gt/volume_0006_0015.png}

&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/deeplab/volume_0006_0015_pred.png_3_636_labeled2-pred_pred.png}

&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/mt/volume_0006_0015_pred.png_7_636_teacher2-pred_pred.png}

&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/advssl/volume_0006_0015.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/gct/volume_0006_0015.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/ours/volume_0006_0015.png}
\\
% \multirow{1}{*}{\rotatebox[origin=c]{90}{NLM}}
\multirow{2}{*}{\rotatebox[origin=c]{90}{MR-T1-out}}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/test-img/volume_0008_0015.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/test-gt/volume_0008_0015.png}
& 
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/deeplab/volume_0008_0015_pred.png_3_134_labeled2-pred_pred.png}
& 
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/mt/volume_0008_0015_pred.png_7_134_teacher2-pred_pred.png}
& 
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/advssl/volume_0008_0015.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/gct/volume_0008_0015.png}

&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/ours/volume_0008_0015.png}

\\
% \multirow{1}{*}{\rotatebox[origin=c]{90}{\scriptsize \hspace{2.7mm}SZ}}
%\rotatebox{90}{\scriptsize \hspace{2.5mm}SZ}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/test-img/volme_0010_0015.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/test-gt/volume_0010_0015.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/deeplab/volume_0010_0015_pred.png_3_388_labeled2-pred_pred.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/mt/volume_0010_0015_pred.png_7_388_teacher2-pred_pred.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/advssl/volume_0010_0015.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/gct/volume_0010_0015.png}
&
\includegraphics[width=0.125\linewidth]{figures/lits/outdomain/ours/volume_0010_0015.png}


\end{tabular}
\end{adjustbox}
\vspace{-4mm}
\caption{\footnotesize \textbf{CT-MRI Liver Segmentation.} Qualitative examples for both in-domain (CT, first row) and out-of-domain (MRI, row 2-5) data. Compared to the baseline methods, \textit{Ours} is more robust to out-of-domain input, which the other methods do not predict well or not at all.}
\label{fig:ct-mri seg}
%\end{minipage}
%\vspace{-6mm}
\end{figure*}

==> figures/results/ct_ssl_eval.tex <==
\begin{table*}[t!]
\vspace{-2.5mm}
\vspace{-1mm}
%\begin{minipage}{0.7\linewidth}
\begin{adjustbox}{width=0.8\linewidth,center}
\rowcolors{2}{white}{gray!15}
\addtolength{\tabcolsep}{-4pt}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
\begin{tabular}{lccccccccccc}
\toprule
 & 
\multicolumn{3}{c}{Trained with \textbf{8} labeled examples} & &
\multicolumn{3}{c}{Trained with \textbf{20} labeled examples} & &
\multicolumn{3}{c}{Trained with \textbf{118} labeled examples} \\
\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
Method& CT & MRI T1-in & MRI T1-out && CT & MRI T1-in & MRI T1-out && CT & MRI T1-in & MRI T1-out \\ 
\midrule
U-Net   & 0.7610 & 0.2568 & 0.3293 && 0.8229 & 0.3428 & 0.2310 && 0.8680 & 0.4453 & 0.4177 \\
DeepLab & 0.7591 & 0.2848 & 0.3286 && 0.8001 & 0.4019 & 0.3798 && 0.9056 & 0.4390 & 0.3767 \\
\midrule

MT                                   & 0.7815 & 0.3589 & 0.0955 &
                                     & 0.8197 & 0.5319 & 0.1908 & 
                                     & 0.8834 & 0.4873 & 0.2596 \\
AdvSSL                               & 0.8005 & 0.5381 & \textbf{0.5855} &
                                     & 0.8105 & 0.5409 & 0.4087 & 
                                     & 0.8551 & 0.4003 & 0.3548 \\
GCT                                  & 0.6997 & 0.4733 & 0.4091 &
                                     & 0.7951 & 0.3469 & \textbf{0.4620} & 
                                     & 0.9085 & 0.4341 & 0.3816 \\
                                     
\midrule                                 
Ours-NO  & 0.8036 & 0.4811 & 0.5135 && 0.8462 & \textbf{0.5538} & 0.4511 && 0.8603 & 0.5055 & \textbf{0.5633} \\
Ours     & \textbf{0.8747} & \textbf{0.5565} & 0.5678 && \textbf{0.8961} & 0.4989 & 0.4575 && \textbf{0.9169} & \textbf{0.5097} & 0.5243 \\
\bottomrule

\end{tabular}
\end{adjustbox}
%\end{minipage}
\hspace{2mm}
%\vspace{-3mm}
%\begin{minipage}{0.282\linewidth}
%\vspace{2mm}
\caption{\footnotesize {\bf CT-MRI Transfer Liver Segmentation.} Numbers are Dice per patient. Here, CT is the in-domain data set on which we both train and evaluate. We also evaluate on additional unseen MRI data~\cite{kavur2020chaos} for liver segmentation. Ours as well as the semi-supervised methods use additional 70 CT volumes from the LITS2017~\cite{bilic2019liver} testing set as unlabeled data samples for training.}
\label{tab:ctmri-ssl}
%\end{minipage}
%\vspace{-6mm}
\end{table*}


==> figures/results/face_classwise_eval_full.tex <==
\begin{table*}[t!]
\begin{adjustbox}{width=0.7\linewidth,center}
\rowcolors{2}{white}{gray!15}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{9}{c}{CelebA-Mask (In-Domain)} \\
\midrule
\rowcolor{white}
Method & Ear & Eye & Eyebrow & Skin & Hair & Mouth & Nose & Mean \\
\midrule
U-Net     & 0.5290 & 0.6608 & 0.6219 & 0.8708 & 0.8129 & 0.7955 & 0.7711 & 0.7231 \\
DeepLab  & 0.6135 & 0.6836 & 0.5911 & 0.8774 & 0.8252 & 0.7957 & 0.8242 & 0.7444 \\

\midrule
MT         & 0.5396 & 0.6586 & 0.5317 & 0.8619 & 0.8104 & 0.7688 & 0.7951 & 0.7094 \\
AdvSSL  & 0.6708 & 0.7254 & \textbf{0.6309} & \textbf{0.8955} & 0.8464 & 0.8376 & \textbf{0.8445} & 0.7787 \\
GCT               & 0.6467 & 0.6991 & 0.6108 & 0.8932 & \textbf{0.8538} & 0.8174 & 0.8408 & 0.7660 \\
\midrule
Ours-NO  & 0.5143 & 0.6770 & 0.5479 & 0.8574 & 0.7937 & 0.7758 & 0.8201 & 0.7123 \\
Ours     & \textbf{0.6968} & \textbf{0.7470} & 0.6150 & 0.8893 & 0.8238 & \textbf{0.8539} & 0.8416 & \textbf{0.7810} \\
\midrule\midrule
\rowcolor{white}
\multicolumn{9}{c}{MetFace-40 (Out-Of-Domain)} \\
\midrule
\rowcolor{white}
Method & Ear & Eye & Eyebrow & Skin & Hair & Mouth & Nose & Mean \\
\midrule
U-Net     & 0.1026 & 0.3393 & 0.3117 & 0.6922 & 0.5347 & 0.4039 & 0.4762 & 0.4086 \\
DeepLab  & 0.2549 & 0.5120 & 0.4026 & 0.8158 & 0.6269 & 0.6155 & 0.7350 & 0.5661 \\
\midrule
MT           & 0.1890 & 0.5135 & 0.3925 & 0.7206 & 0.5266 & 0.5663 & 0.6837 & 0.5132 \\
AdvSSL    & 0.3241 & 0.5340 & 0.4236 & 0.8345 & 0.6556 & 0.6642 & 0.7604 & 0.5995 \\
GCT              & 0.2467 & 0.5486 & 0.4393 & 0.8434 & 0.6753 & 0.6744 & 0.7563 & 0.5977 \\
\midrule
Ours-NO  & 0.2795 & 0.5422 & 0.3880 & 0.8114 & 0.6370 & 0.6173 & 0.7492 & 0.5749 \\
Ours     & \textbf{0.5224} & \textbf{0.6025} & \textbf{0.4810} & \textbf{0.8534} & \textbf{0.6995} & \textbf{0.6957} & \textbf{0.7915} & \textbf{0.6633} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{3mm}
\caption{\footnotesize \textbf{CelebA-Mask Segmentation Results using 1500 Labels during Training.} CelebA-Mask segmentation results for different face parts for in-domain data (real faces, top part) and for out-of-domain data (MetFaces, bottom part).}
\label{tab:celeba-classwise-full}
\end{table*}

==> figures/results/face_classwise_eval_large.tex <==
\begin{table*}[h!]
\begin{adjustbox}{width=0.7\linewidth,center}
\rowcolors{2}{white}{gray!15}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{9}{c}{CelebA-Mask (In-Domain)} \\
\midrule
\rowcolor{white}
Method & Ear & Eye & Eyebrow & Skin & Hair & Mouth & Nose & Mean \\
\midrule
U-Net     & 0.5095 & 0.5686 & 0.6040 & 0.8414 & 0.7790 & 0.7627 & 0.7513 & 0.6880 \\
DeepLab  & 0.4313 & 0.6308 & 0.4905 & 0.8317 & 0.7392 & 0.7174 & 0.7729 & 0.6591 \\

\midrule
MT       & 0.4125 & 0.4946 & 0.4035 & 0.7969 & 0.7370 & 0.6398 & 0.6153 & 0.5857 \\
AdvSSL  & 0.4902 & 0.6465 & 0.5103 & 0.8517 & 0.7567 & 0.7453 & 0.7912 & 0.6846 \\
GCT          & 0.4411 & 0.5714 & 0.3623 & 0.8502 & 0.7977 & 0.6965 & 0.7631 & 0.6403 \\
\midrule
Ours-NO  & 0.5064 & 0.6474 & 0.5437 & 0.8516 & 0.7834 & 0.7601 & 0.8183 & 0.7016 \\
Ours     & \textbf{0.6722} & \textbf{0.6900} & \textbf{0.6101} & \textbf{0.8798} & \textbf{0.8164} & \textbf{0.8173} & \textbf{0.8343} & \textbf{0.7600} \\
\midrule\midrule
\rowcolor{white}
\multicolumn{9}{c}{MetFace-40 (Out-Of-Domain)} \\
\midrule
\rowcolor{white}
Method & Ear & Eye & Eyebrow & Skin & Hair & Mouth & Nose & Mean \\
\midrule
U-Net     & 0.1036 & 0.1568 & 0.2371 & 0.4840 & 0.3718 & 0.2272 & 0.3817 & 0.2803 \\
DeepLab  & 0.1804 & 0.4882 & 0.3494 & 0.7437 & 0.5372 & 0.5491 & 0.6434 & 0.4988 \\
\midrule
MT         & 0.2217 & 0.2709 & 0.2603 & 0.6986 & 0.5048 & 0.5031 & 0.5537 & 0.4305 \\
AdvSSL    & 0.1913 & 0.4663 & 0.3184 & 0.7374 & 0.5620 & 0.5745 & 0.6708 & 0.5029 \\
GCT              & 0.1014 & 0.3530 & 0.1819 & 0.7898 & 0.6430 & 0.5838 & 0.6715 & 0.4749 \\
\midrule
Ours-NO  & 0.2845 & 0.5260 & 0.4011 & 0.8000 & 0.6141 & 0.6108 & 0.7133 & 0.5643 \\
Ours     & \textbf{0.5030} & \textbf{0.5517} & \textbf{0.4226} & \textbf{0.8459} & \textbf{0.6810} & \textbf{0.6702} & \textbf{0.7612} & \textbf{0.6336} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{3mm}
\caption{\footnotesize \textbf{CelebA-Mask Segmentation Results using 150 Labels during Training.} CelebA-Mask segmentation results for different face parts for in-domain data (real faces, top part) and for out-of-domain data (MetFaces, bottom part).}
\label{tab:celeba-classwise-large}
\end{table*}

==> figures/results/face_classwise_eval_small.tex <==
\begin{table*}[h!]
\begin{adjustbox}{width=0.7\linewidth,center}
\rowcolors{2}{white}{gray!15}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{9}{c}{CelebA-Mask (In-Domain)} \\
\midrule
\rowcolor{white}
Method & Ear & Eye & Eyebrow & Skin & Hair & Mouth & Nose & Mean \\
\midrule
U-Net     & 0.3381 & 0.4429 & 0.5138 & 0.7575 & 0.7022 & 0.5988 & 0.5259 & 0.5764 \\
DeepLab  & 0.2706 & 0.4828 & 0.3921 & 0.7746 & 0.6654 & 0.6308 & 0.6718 & 0.5554 \\

\midrule
MT       & 0.0000 & 0.0000 & 0.0000 & 0.5699 & 0.1860 & 0.0004 & 0.0010 & 0.1082 \\
AdvSSL   & 0.2908 & 0.3275 & 0.3945 & 0.7572 & \textbf{0.5932} & 0.6094 & 0.6271 & 0.5142 \\
GCT            & 0.1317 & 0.1926 & 0.0295 & 0.6866 & 0.5565 & 0.4520 & 0.5366 & 0.3694 \\
\midrule
Ours-NO  & 0.4855 & 0.6004 & 0.5403 & 0.8383 & 0.5659 & 0.7139 & 0.7872 & 0.6473 \\
Ours     & \textbf{0.6400} & \textbf{0.6069} & \textbf{0.6071} & \textbf{0.8531} & 0.5878 & \textbf{0.7437} & \textbf{0.7925} & \textbf{0.6902} \\
\midrule\midrule
\rowcolor{white}
\multicolumn{9}{c}{MetFace-40 (Out-Of-Domain)} \\
\midrule
\rowcolor{white}
Method & Ear & Eye & Eyebrow & Skin & Hair & Mouth & Nose & Mean \\
\midrule
U-Net     & 0.1036 & 0.1568 & 0.2371 & 0.4840 & 0.3718 & 0.2272 & 0.3817 & 0.2803 \\
DeepLab  & 0.1016 & 0.3957 & 0.2479 & 0.6569 & 0.4784 & 0.5052 & 0.5975 & 0.4262 \\

\midrule
MT        & 0.0000 & 0.0000 & 0.0000 & 0.6157 & 0.3737 & 0.0000 & 0.0009 & 0.1415 \\
AdvSSL    & 0.1247 & 0.1624 & 0.2526 & 0.7014 & 0.4795 & 0.4956 & 0.6018 & 0.4026 \\
GCT            & 0.0421 & 0.1247 & 0.0192 & 0.5929 & 0.3976 & 0.4095 & 0.5403 & 0.3038 \\
\midrule
Ours-NO  & 0.2982 & \textbf{0.4986} & 0.3972 & 0.8114 & \textbf{0.5502} & 0.6034 & 0.6953 & 0.5506 \\
Ours     & \textbf{0.4395} & 0.4674 & \textbf{0.4704} & \textbf{0.8293} & 0.5452 & \textbf{0.6581} & \textbf{0.7082} & \textbf{0.5883} \\
\bottomrule

\end{tabular}
\end{adjustbox}
\vspace{3mm}
\caption{\footnotesize \textbf{CelebA-Mask Segmentation Results using 30 Labels during Training.} CelebA-Mask segmentation results for different face parts for in-domain data (real faces, top part) and for out-of-domain data (MetFaces, bottom part).}
\label{tab:celeba-classwise-small}
\end{table*}


==> figures/results/other.tex <==
\begin{table*}[p!]
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
Dataset & Train & Test \\ \hline\hline
JSRT/SCR \cite{shiraishi2000development,van2006segmentation}& 175 & 72\\
Chestxray-14 \cite{wang2017chestx} &108K & - \\
NLM(MC) \cite{jaeger2014two} & - & 138\\
NLM(Shenzhen) \cite{jaeger2014two, stirenko2018chest} & - & 566\\
NIH \cite{tang2019xlsor} & - & 100\\
\hline
\end{tabular}
\end{center}
\caption{Chest X-ray Lung Segmentation Datasets}
\label{tab:xray-dataset}
\end{table*}

% \begin{table*}[p!]
% \begin{adjustbox}{width=\columnwidth,center}

% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
%  & 
% \multicolumn{2}{c|}{Size 9} & 
% \multicolumn{2}{c|}{Size 35} &
% \multicolumn{2}{c|}{Size 175} \\
% \hline
% Method& DSC & ASSD & DSC & ASSD & DSC & ASSD \\ 
% \hline\hline
% U-Net     & 0.9318 & 2.93 & 0.9308 & 2.99 & 0.9464 & 2.28 \\
% nnU-Net   & 0.9672 & 1.38 & 0.9769 & 1.03 & 0.9796 & 0.88 \\
% \hline
% BS1       & - & - & - & - & - & - \\
% BS2       & - & - & - & - & - & - \\
% Ours-NO   & 0.9464 & 1.88 & 0.9471 & 2.17 & 0.9465 & 2.17 \\
% Ours      & 0.9591 & 1.70 & 0.9668 & 1.40 & 0.9669 & 1.39 \\
% \hline

% \end{tabular}
% \end{adjustbox}
% \vspace{3mm}
% \caption{Chest X-ray Lung Segmentation in-domain results}
% \label{tab:xray-in-domain}

% \end{table*}

% MOVED
% \begin{table*}[t!]
% \begin{adjustbox}{width=\textwidth,center}

% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
%  & 
% \multicolumn{4}{c|}{Size 9} & 
% \multicolumn{4}{c|}{Size 35} &
% \multicolumn{4}{c|}{Size 175} \\
% \hline
% Method& CXR14 & NLM & NIH & SZ & CXR14 & NLM & NIH & SZ & CXR14 & NLM & NIH & SZ \\ 
% \hline\hline
% U-Net            & 0.9318 & 0.8605 & 0.6801 & 0.9051 
%                 & 0.9308 & 0.8591 & 0.7363 & 0.8486 
%                 & 0.9464 & 0.9143 & 0.7553 & 0.9005\\
                
% nnU-Net          & \textbf{0.9672} & 0.9290 & 0.7559 & 0.9114 
%                 & \textbf{0.9769} & 0.9317 & 0.8255 & 0.9345 
%                 & \textbf{0.9796} & 0.9484 & 0.8526 & \textbf{0.9497}\\
                
% DeepLab         & 0.9006 & 0.6324 & 0.7361 & 0.8124 
%                 & 0.9556 & 0.8323 & 0.8099 & 0.9138 
%                 & 0.9666 & 0.8175 & 0.8093 & 0.9312\\
                
% \hline
% MT \cite{tarvainen2017mean}          & 0.9239 & 0.8287 & 0.7280 & 0.8847 
%                                      & 0.9436 & 0.8239 & 0.7305 & 0.8306 
%                                      & 0.9604 & 0.8626 & 0.7893 & 0.8846 \\
                                     
% AdvSSL \cite{hung2018adversarial}    & 0.9328 & 0.8500 & 0.7720 & 0.8901 
%                                      & 0.9552 & 0.8191 & 0.5298 & 0.8968 
%                                      & 0.9684 & 0.8344 & 0.7627 & 0.8846 \\
                                     
% GCT \cite{ke2020guided}              & 0.9235 & 0.6804 & 0.6731 & 0.8665 
%                                      & 0.9502 & 0.8327 & 0.7527 & 0.9184 
%                                      & 0.9644 & 0.4482 & 0.7981 & 0.9393 \\

% \hline

% Ours-NO  & 0.9464 & 0.9303 & 0.9097 & 0.9334 & 0.9471 & 0.9294 & 0.9223 & 0.9409 & 0.9465 & 0.9232 & 0.9204 & 0.9403 \\
% Ours     & 0.9591 & \textbf{0.9464} & \textbf{0.9133} & \textbf{0.9362} & 0.9668 & \textbf{0.9606} & \textbf{0.9322} & \textbf{0.9485} & 0.9669 & \textbf{0.9509} & \textbf{0.9294} & 0.9469 \\
% \hline

% \end{tabular}
% \end{adjustbox}
% \vspace{3mm}
% \caption{Chest X-ray Lung Segmentation out-domain results}
% \label{tab:xray-out-domain}

% \end{table*}


%----------------------------------------------------------------------------------------------------%

% \subsection{Skin Lesion segmentation}
% In this experiment we use \textit{ISIC2020} as unlabeled dataset $D_u$ and \textit{ISIC2018} as labeled dataset $D_l$ (see Table ~\ref{tab:skin-dataset}) to compare segmentation in-domain performance. We use the other three datasets \textit{$PH^2$}, \textit{DermIS} and \textit{DermQuest} as out-domain test.

% \subsubsection{In-domain evaluation}

% \subsubsection{Out-domain evaluation}

\begin{table*}[p!]
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
Dataset & Train & Test \\ \hline\hline
ISIC2018 \cite{codella2019skin,van2006segmentation}& 2000 & 594\\
ISIC2020 \cite{rotemberg2020patientcentric} & 33126 & - \\
PH2 \cite{mendoncca2013ph} & - & 200\\
DermIS \cite{?} & - & 69\\
DermQuest \cite{?} & - & 98\\
\hline
\end{tabular}
\end{center}
\caption{Skin Lesion Segmentation Dataset}
\label{tab:skin-dataset}
\end{table*}

% \begin{table*}[t!]
% \begin{adjustbox}{width=\columnwidth,center}

% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
%  & 
% \multicolumn{2}{c|}{Size 40} & 
% \multicolumn{2}{c|}{Size 200} &
% \multicolumn{2}{c|}{Size 2000} \\
% \hline
% Method& JC & ASSD & JC & ASSD & JC & ASSD \\ 
% \hline\hline
% U-Net     & 0.4069 & - & 0.6638 & - & 0.6817 & - \\
% DeepLab  & 0.6148 & - & 0.7432 & - & 0.7448 & - \\
% \hline
% BS1      & - & - & - & - & - & - \\
% BS2      & - & - & - & - & - & - \\
% Ours-NO  & 0.7092 & - & 0.7709 & - & 0.7841 & - \\
% Ours     & 0.7357 & - & 0.7673 & - & 0.7906 & - \\
% \hline

% \end{tabular}
% \end{adjustbox}
% \vspace{3mm}
% \caption{ISIC Skin Lesion Segmentation in-domain results}
% \label{tab:isic-in-domain}
% \end{table*}


%----------------------------------------------------------------------------------------------------%

% \subsection{CT-MRI Cross-modality Liver segmentation}
% In this experiment we use \textit{LITS2017-test} as unlabeled dataset $D_u$ and \textit{LITS2017-train} as labeled dataset $D_l$ (see Table ~\ref{tab:ct-mri-dataset}) to compare segmentation in-domain performance. We use the other two datasets \textit{CHAOS-T1-in}, and \textit{CHAOS-T1-out} as out-domain test.

% \subsubsection{In-domain evaluation}

% \subsubsection{Out-domain evaluation}
\begin{table*}[p!]
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
Dataset & Train & Test \\ \hline\hline
CelebA-mask-l \cite{CelebAMask-HQ}& 1500 & 500\\
CelebA-mask-u \cite{CelebAMask-HQ} & 28000 & -\\
MetFaces \cite{karras2020training} & - & 40\\
%WebCaricature \cite{Huo:2017:VRC:3126686.3126736, HuoBMVC2018WebCaricature} & - & 100\\
\hline
\end{tabular}
\end{center}
\caption{Face Parts Segmentation Dataset.}
\label{tab:face-dataset}
\vspace{-3mm}
\end{table*}


\begin{table*}[p!]
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
Dataset & Train & Test \\ \hline\hline
LITS2017-train \cite{bilic2019liver}& 118 & 13\\
LITS2017-test \cite{bilic2019liver} & 70  & -\\
CHAOS-T1-in \cite{kavur2020chaos, kavur2019, CHAOSdata2019} & - & 20\\
CHAOS-T1-out \cite{kavur2020chaos, kavur2019, CHAOSdata2019} & - & 20\\
\hline
\end{tabular}
\end{center}
\caption{CT-MRI Liver Segmentation Dataset. Number of Patients.}
\label{tab:ct-mri-dataset}
\end{table*}
